Joint Distribution-Informed Shapley Values for Sparse Counterfactual Explanations

Counterfactual explanations (CE) aim to reveal how small input changes flip a model's prediction, yet many methods modify more features than necessary, reducing clarity and actionability. We introduce \emph{COLA}, a model- and generator-agnostic post-hoc framework that refines any given CE by computing a coupling via optimal transport (OT) between factual and counterfactual sets and using it to drive a Shapley-based attribution (\emph{$p$-SHAP}) that selects a minimal set of edits while preserving the target effect. Theoretically, OT minimizes an upper bound on the $W_1$ divergence between factual and counterfactual outcomes and that, under mild conditions, refined counterfactuals are guaranteed not to move farther from the factuals than the originals. Empirically, across four datasets, twelve models, and five CE generators, COLA achieves the same target effects with only 26--45\% of the original feature edits. On a small-scale benchmark, COLA shows near-optimality.

==> pictures/cola_illustration.tex <==



\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,793); %set diagram left start at 0, and has height of 793

%Shape: Rectangle [id:dp7535053490619492] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][dash pattern={on 4.5pt off 4.5pt}][line width=0.75]  (12.4,423.84) -- (142.2,423.84) -- (142.2,537.8) -- (12.4,537.8) -- cycle ;
%Shape: Rectangle [id:dp08263773607739133] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][dash pattern={on 4.5pt off 4.5pt}][line width=0.75]  (144.2,423.84) -- (276.2,423.84) -- (276.2,537.8) -- (144.2,537.8) -- cycle ;
%Straight Lines [id:da31439005867812875] 
\draw [color={rgb, 255:red, 249; green, 1; blue, 1 }  ,draw opacity=1 ]   (186.24,456.19) -- (230.47,449.15) ;
%Straight Lines [id:da3123340329661606] 
\draw [color={rgb, 255:red, 249; green, 1; blue, 1 }  ,draw opacity=1 ]   (186.24,456.19) -- (230.47,464.64) ;
%Straight Lines [id:da5960824802628599] 
\draw [color={rgb, 255:red, 249; green, 1; blue, 1 }  ,draw opacity=1 ]   (186.24,474.49) -- (230.47,464.64) ;
%Straight Lines [id:da391228469232932] 
\draw [color={rgb, 255:red, 249; green, 1; blue, 1 }  ,draw opacity=1 ]   (186.24,474.49) -- (230.89,481.18) ;
%Shape: Rectangle [id:dp5253464464390294] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][dash pattern={on 4.5pt off 4.5pt}][line width=0.75]  (278.2,423.84) -- (409.2,423.84) -- (409.2,537.8) -- (278.2,537.8) -- cycle ;
%Straight Lines [id:da5394277178144502] 
\draw [color={rgb, 255:red, 249; green, 1; blue, 1 }  ,draw opacity=1 ][line width=1.5]    (319.25,456.19) -- (363.47,449.15) ;
%Straight Lines [id:da5344835720127035] 
\draw [color={rgb, 255:red, 249; green, 1; blue, 1 }  ,draw opacity=1 ][line width=1.5]    (319.25,474.49) -- (363.9,481.18) ;
%Shape: Rectangle [id:dp014762474359765632] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][dash pattern={on 4.5pt off 4.5pt}][line width=0.75]  (411.2,423.84) -- (539.8,423.84) -- (539.8,537.3) -- (411.2,537.3) -- cycle ;
%Shape: Circle [id:dp9888883013739482] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ] (230.47,464.64) .. controls (230.47,460.92) and (233.48,457.9) .. (237.2,457.9) .. controls (240.92,457.9) and (243.93,460.92) .. (243.93,464.64) .. controls (243.93,468.35) and (240.92,471.37) .. (237.2,471.37) .. controls (233.48,471.37) and (230.47,468.35) .. (230.47,464.64) -- cycle ;
%Shape: Circle [id:dp42655365148405355] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ] (230.47,449.15) .. controls (230.47,445.43) and (233.48,442.42) .. (237.2,442.42) .. controls (240.92,442.42) and (243.93,445.43) .. (243.93,449.15) .. controls (243.93,452.87) and (240.92,455.88) .. (237.2,455.88) .. controls (233.48,455.88) and (230.47,452.87) .. (230.47,449.15) -- cycle ;
%Shape: Circle [id:dp04025310028865525] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ] (230.89,481.18) .. controls (230.89,477.46) and (233.91,474.45) .. (237.63,474.45) .. controls (241.34,474.45) and (244.36,477.46) .. (244.36,481.18) .. controls (244.36,484.9) and (241.34,487.91) .. (237.63,487.91) .. controls (233.91,487.91) and (230.89,484.9) .. (230.89,481.18) -- cycle ;
%Shape: Circle [id:dp4413090996175171] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ] (172.78,456.19) .. controls (172.78,452.47) and (175.79,449.46) .. (179.51,449.46) .. controls (183.23,449.46) and (186.24,452.47) .. (186.24,456.19) .. controls (186.24,459.91) and (183.23,462.92) .. (179.51,462.92) .. controls (175.79,462.92) and (172.78,459.91) .. (172.78,456.19) -- cycle ;
%Shape: Circle [id:dp05666246265076169] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ] (172.78,474.49) .. controls (172.78,470.77) and (175.79,467.76) .. (179.51,467.76) .. controls (183.23,467.76) and (186.24,470.77) .. (186.24,474.49) .. controls (186.24,478.21) and (183.23,481.22) .. (179.51,481.22) .. controls (175.79,481.22) and (172.78,478.21) .. (172.78,474.49) -- cycle ;
%Shape: Circle [id:dp1875745396004196] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ] (305.78,456.19) .. controls (305.78,452.47) and (308.8,449.46) .. (312.52,449.46) .. controls (316.23,449.46) and (319.25,452.47) .. (319.25,456.19) .. controls (319.25,459.91) and (316.23,462.92) .. (312.52,462.92) .. controls (308.8,462.92) and (305.78,459.91) .. (305.78,456.19) -- cycle ;
%Shape: Circle [id:dp3994303283770062] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ] (305.78,474.49) .. controls (305.78,470.77) and (308.8,467.76) .. (312.52,467.76) .. controls (316.23,467.76) and (319.25,470.77) .. (319.25,474.49) .. controls (319.25,478.21) and (316.23,481.22) .. (312.52,481.22) .. controls (308.8,481.22) and (305.78,478.21) .. (305.78,474.49) -- cycle ;
%Shape: Circle [id:dp48800034099409584] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ] (363.47,449.15) .. controls (363.47,445.43) and (366.49,442.42) .. (370.21,442.42) .. controls (373.92,442.42) and (376.94,445.43) .. (376.94,449.15) .. controls (376.94,452.87) and (373.92,455.88) .. (370.21,455.88) .. controls (366.49,455.88) and (363.47,452.87) .. (363.47,449.15) -- cycle ;
%Shape: Circle [id:dp8625213418870858] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ] (363.97,464.65) .. controls (363.97,460.93) and (366.99,457.92) .. (370.71,457.92) .. controls (374.42,457.92) and (377.44,460.93) .. (377.44,464.65) .. controls (377.44,468.37) and (374.42,471.38) .. (370.71,471.38) .. controls (366.99,471.38) and (363.97,468.37) .. (363.97,464.65) -- cycle ;
%Shape: Circle [id:dp7144402341162441] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ] (363.9,481.18) .. controls (363.9,477.46) and (366.92,474.45) .. (370.63,474.45) .. controls (374.35,474.45) and (377.37,477.46) .. (377.37,481.18) .. controls (377.37,484.9) and (374.35,487.91) .. (370.63,487.91) .. controls (366.92,487.91) and (363.9,484.9) .. (363.9,481.18) -- cycle ;
%Shape: Rectangle [id:dp8245410288318857] 
\draw  [draw opacity=0][fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (203.2,446.02) -- (223.2,446.02) -- (223.2,457.8) -- (203.2,457.8) -- cycle ;

%Shape: Rectangle [id:dp21975854625333935] 
\draw  [draw opacity=0][fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (203.2,457.9) -- (223.2,457.9) -- (223.2,473.98) -- (203.2,473.98) -- cycle ;

%Shape: Rectangle [id:dp8570022291981747] 
\draw  [draw opacity=0][fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (203.2,475.52) -- (223.2,475.52) -- (223.2,487.3) -- (203.2,487.3) -- cycle ;


% Text Node
\draw (27.07,507.22) node [anchor=north west][inner sep=0.75pt]    {$\textcolor[rgb]{0.93,0.04,0.04}{\vec{p}}( \vec{x},\textcolor[rgb]{0.29,0.56,0.89}{\vec{r}})\leftarrow A_{\text{Prob}}$};
% Text Node
\draw (83.08,441.98) node [anchor=north west][inner sep=0.75pt]    {$\textcolor[rgb]{0.29,0.56,0.89}{\vec{r}}\leftarrow A_{\text{CE}}$};
% Text Node
\draw (46.62,537.36) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {Lines 1--2};
% Text Node
\draw (180.34,537.36) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {Lines 3--4};
% Text Node
\draw (38.13,455.25) node [anchor=north west][inner sep=0.75pt]    {$\vec{x}$};
% Text Node
\draw (176.13,483.6) node [anchor=north west][inner sep=0.75pt]    {$\textcolor[rgb]{0.25,0.46,0.02}{\bm{\varphi} }\leftarrow A_{\text{Shap}}$};
% Text Node
\draw (189.31,460.34) node [anchor=north west][inner sep=0.75pt]    {$\textcolor[rgb]{0.96,0.03,0.03}{\vec{p}}$};
% Text Node
\draw (162.16,461.25) node [anchor=north west][inner sep=0.75pt]    {$\vec{x}$};
% Text Node
\draw (244.28,461.25) node [anchor=north west][inner sep=0.75pt]    {$\textcolor[rgb]{0.29,0.56,0.89}{\vec{r}}$};
% Text Node
\draw (321.94,537.36) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {Line 5};
% Text Node
\draw (303.29,483) node [anchor=north west][inner sep=0.75pt]    {$\textcolor[rgb]{0.56,0.07,1}{\vec{q}}\leftarrow A_{\text{Value}}^{\text{max}}$};
% Text Node
\draw (295.17,461.25) node [anchor=north west][inner sep=0.75pt]    {$\vec{x}$};
% Text Node
\draw (377.29,461.25) node [anchor=north west][inner sep=0.75pt]    {$\textcolor[rgb]{0.29,0.56,0.89}{\vec{r}}$};
% Text Node
\draw (321.26,460.19) node [anchor=north west][inner sep=0.75pt]    {$\textcolor[rgb]{0.96,0.03,0.03}{\vec{p}}$};
% Text Node
\draw (446.07,537.36) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {Lines 6--16};
% Text Node
\draw (11.41,464.72) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize]  {$\begin{bmatrix}
x_{11} & x_{12}\\
x_{21} & x_{22}
\end{bmatrix}$};
% Text Node
\draw (74.66,455.69) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ]  {$\begin{bmatrix}
r_{11} & r_{12}\\
r_{21} & r_{22}\\
r_{31} & r_{32}
\end{bmatrix}$};
% Text Node
\draw (155.88,499.93) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize,color={rgb, 255:red, 65; green, 117; blue, 5 }  ,opacity=1 ]  {$\bm{\varphi} =\begin{bmatrix}
\varphi _{11} & \varphi _{12}\\
\varphi _{21} & \varphi _{22}
\end{bmatrix}$};
% Text Node
\draw (296.87,500.89) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize,color={rgb, 255:red, 144; green, 19; blue, 254 }  ,opacity=1 ]  {$\vec{q}=\begin{bmatrix}
r_{11} & r_{12}\\
r_{31} & r_{32}
\end{bmatrix}$};
% Text Node
\draw (419.17,501.79) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize]  {$\rightarrow \vec{z}=\begin{bmatrix}
x_{11} & \textcolor[rgb]{0.56,0.07,1}{q}\textcolor[rgb]{0.56,0.07,1}{_{12}}\\
\textcolor[rgb]{0.56,0.07,1}{q}\textcolor[rgb]{0.56,0.07,1}{_{21}} & x_{22}
\end{bmatrix}$};
% Text Node
\draw (410.54,437.67) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 65; green, 117; blue, 5 }  ,opacity=1 ]  {$\begin{bmatrix}
\varphi _{11} =0.2 & \varphi _{12} =0.4\\
\varphi _{21} =0.3 & \varphi _{22} =0.1
\end{bmatrix}$};
% Text Node
\draw (412.24,469.82) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize]  {$ \begin{array}{l}
C=2\\
\rightarrow \vec{c}\sim\{( 1,2) , (2,1)\}
\end{array}$};
% Text Node
\draw (11.4,423.8) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\small Obtain $\vec{r}$ and compute $\vec{p}$}};
% Text Node
\draw (145.55,423.8) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\small Use $\displaystyle \vec{p}$ to compute Shapley}};
% Text Node
\draw (278.56,423.8) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\small Match $\displaystyle \vec{x}_{i}$ to $\displaystyle \vec{r}_{\text{argmax}_{j} p( \vec{r}_{j} |\vec{x}_{i})}$}};
% Text Node
\draw (411.85,423.3) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {{\small Get $\displaystyle \vec{c}$ and $\displaystyle \vec{z}$ by $\displaystyle \bm{\varphi} $ and $\displaystyle \vec{q}$}};
% Text Node
\draw (203.2,473.86) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$\textcolor[rgb]{0.97,0.03,0.03}{0.3}$};
% Text Node
\draw (203.2,458.54) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$\textcolor[rgb]{0.97,0.02,0.02}{0.1}$};
% Text Node
\draw (203.2,444.36) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$\textcolor[rgb]{0.97,0.02,0.02}{0.5}$};


\end{tikzpicture}

==> pictures/german_credit_optimality/adaboost_DiCE.tex <==

\begin{tikzpicture}
\begin{axis}[
    width=4.4cm, height=3.6cm,
    legend pos=north east,
    legend style={
        draw=none,
        % font=\scriptsize,
        legend image code/.code={
            \draw[mark repeat=2,mark phase=2]
                plot coordinates {
                    (0cm,0cm)
                    (0.4cm,0cm) % Adjust the length here
                };
        },
        inner xsep=0pt, % Adjust inner x separation
        inner ysep=0pt  % Adjust inner y separation
    },
    legend cell align={left},
    grid=major,
    title={AdaBoost, $\A_{\text{CE}}=$DiCE},
    title style={font=\footnotesize, yshift=-1ex}, 
    font=\footnotesize,
    % Increase margin of x and y tick labels
    xticklabel style={xshift=-0pt, yshift=-3pt},
    yticklabel style={xshift=-3pt, yshift=0pt},
]
        \addplot[name path=CF-OT-MeanD-line, red, solid] coordinates {
    (0, 0.8599999999999995)
    (5, 0.7742000000000003)
    (10, 0.6974000000000002)
    (15, 0.6297999999999995)
    (20, 0.5516)
    (25, 0.49099999999999966)
    (30, 0.42900000000000027)
    (35, 0.36780000000000007)
    (40, 0.3180000000000001)
    (45, 0.2538000000000002)
    (50, 0.21439999999999995)
    (55, 0.15839999999999999)
    (60, 0.10939999999999994)
    (65, 0.07419999999999995)
    (70, 0.03400000000000002)
    (75, 0.010400000000000005)
    (80, 0.0)
    (85, 0.0)
    (90, 0.0)
    (95, 0.0)
    (100, 0.0)
    (105, 0.0)
    (110, 0.0)
    (115, 0.0)
    (120, 0.0)
    (125, 0.0)
    (130, 0.0)
    (135, 0.0)
    (140, 0.0)
    (145, 0.0)
    (150, 0.0)
    (155, 0.0)
    (160, 0.0)
    (165, 0.0)
    (170, 0.0)
    (175, 0.0)
    (180, 0.0)
    (185, 0.0)
    (190, 0.0)
    (195, 0.0)
    (200, 0.0)
};
%\addlegendentry{CF-OT}
\addplot[name path=CF-OT-MeanD-upper, red, opacity=0.3, forget plot] coordinates {
    (0, 0.8599999999999997)
    (5, 0.7789731981471131)
    (10, 0.7051127447983454)
    (15, 0.6387037212808797)
    (20, 0.5615464452206002)
    (25, 0.5019891807315192)
    (30, 0.441042542031897)
    (35, 0.3793474244833903)
    (40, 0.331343777412712)
    (45, 0.2646431333415948)
    (50, 0.22643192480521712)
    (55, 0.16947967827720642)
    (60, 0.11970056713722108)
    (65, 0.08384189988703467)
    (70, 0.0406148281338218)
    (75, 0.014813377018837165)
    (80, 0.0)
    (85, 0.0)
    (90, 0.0)
    (95, 0.0)
    (100, 0.0)
    (105, 0.0)
    (110, 0.0)
    (115, 0.0)
    (120, 0.0)
    (125, 0.0)
    (130, 0.0)
    (135, 0.0)
    (140, 0.0)
    (145, 0.0)
    (150, 0.0)
    (155, 0.0)
    (160, 0.0)
    (165, 0.0)
    (170, 0.0)
    (175, 0.0)
    (180, 0.0)
    (185, 0.0)
    (190, 0.0)
    (195, 0.0)
    (200, 0.0)
};
\addplot[name path=CF-OT-MeanD-lower, red, opacity=0.3, forget plot] coordinates {
    (0, 0.8599999999999994)
    (5, 0.7694268018528876)
    (10, 0.6896872552016551)
    (15, 0.6208962787191192)
    (20, 0.5416535547793998)
    (25, 0.4800108192684801)
    (30, 0.4169574579681035)
    (35, 0.3562525755166098)
    (40, 0.30465622258728825)
    (45, 0.2429568666584056)
    (50, 0.20236807519478278)
    (55, 0.14732032172279355)
    (60, 0.09909943286277881)
    (65, 0.06455810011296523)
    (70, 0.02738517186617825)
    (75, 0.005986622981162844)
    (80, 0.0)
    (85, 0.0)
    (90, 0.0)
    (95, 0.0)
    (100, 0.0)
    (105, 0.0)
    (110, 0.0)
    (115, 0.0)
    (120, 0.0)
    (125, 0.0)
    (130, 0.0)
    (135, 0.0)
    (140, 0.0)
    (145, 0.0)
    (150, 0.0)
    (155, 0.0)
    (160, 0.0)
    (165, 0.0)
    (170, 0.0)
    (175, 0.0)
    (180, 0.0)
    (185, 0.0)
    (190, 0.0)
    (195, 0.0)
    (200, 0.0)
};
\addplot[fill opacity=0.3, red, forget plot] fill between[of=CF-OT-MeanD-upper and CF-OT-MeanD-lower];
\addplot[name path=CF_Exact-MeanD-line, black, dashed] coordinates {
    (0, 0.8599999999999995)
    (5, 0.7712000000000007)
    (10, 0.6803999999999999)
    (15, 0.5993999999999997)
    (20, 0.518)
    (25, 0.4420000000000001)
    (30, 0.36099999999999993)
    (35, 0.28040000000000026)
    (40, 0.20919999999999983)
    (45, 0.13720000000000002)
    (50, 0.06819999999999996)
    (55, 0.013600000000000008)
    (60, 0.0)
    (65, 0.0)
    (70, 0.0)
    (75, 0.0)
    (80, 0.0)
    (85, 0.0)
    (90, 0.0)
    (95, 0.0)
    (100, 0.0)
    (105, 0.0)
    (110, 0.0)
    (115, 0.0)
    (120, 0.0)
    (125, 0.0)
    (130, 0.0)
    (135, 0.0)
    (140, 0.0)
    (145, 0.0)
    (150, 0.0)
    (155, 0.0)
    (160, 0.0)
    (165, 0.0)
    (170, 0.0)
    (175, 0.0)
    (180, 0.0)
    (185, 0.0)
    (190, 0.0)
    (195, 0.0)
    (200, 0.0)
};
%\addlegendentry{CF_Exact}
\addplot[name path=Optimal-MeanD-line, black, solid] coordinates {
    (0, 0.8599998950958252)
    (5, 0.76)
    (10, 0.6600000000000003)
    (15, 0.5600000000000002)
    (20, 0.46000000000000013)
    (25, 0.36000000000000004)
    (30, 0.25999999999999995)
    (35, 0.16)
    (40, 0.06)
    (45, 0.0)
    (50, 0.0)
    (55, 0.0)
    (60, 0.0)
    (65, 0.0)
    (70, 0.0)
    (75, 0.0)
    (80, 0.0)
    (85, 0.0)
    (90, 0.0)
    (95, 0.0)
    (100, 0.0)
    (105, 0.0)
    (110, 0.0)
    (115, 0.0)
    (120, 0.0)
    (125, 0.0)
    (130, 0.0)
    (135, 0.0)
    (140, 0.0)
    (145, 0.0)
    (150, 0.0)
    (155, 0.0)
    (160, 0.0)
    (165, 0.0)
    (170, 0.0)
    (175, 0.0)
    (180, 0.0)
    (185, 0.0)
    (190, 0.0)
    (195, 0.0)
    (200, 0.0)
};
%\addlegendentry{Optimal}
\end{axis}
\end{tikzpicture}



==> pictures/german_credit_optimality/dnn_KNN.tex <==

\begin{tikzpicture}
\begin{axis}[
    width=4.4cm, height=3.6cm,
    legend pos=north east,
    legend style={
        draw=none,
        % font=\scriptsize,
        legend image code/.code={
            \draw[mark repeat=2,mark phase=2]
                plot coordinates {
                    (0cm,0cm)
                    (0.4cm,0cm) % Adjust the length here
                };
        },
        inner xsep=0pt, % Adjust inner x separation
        inner ysep=0pt  % Adjust inner y separation
    },
    legend cell align={left},
    grid=major,
    title={DNN, $\A_{\text{CE}}=$KNN},
    title style={font=\footnotesize, yshift=-1ex}, 
    font=\footnotesize,
    % Increase margin of x and y tick labels
    xticklabel style={xshift=-0pt, yshift=-3pt},
    yticklabel style={xshift=-3pt, yshift=0pt},
]
        \addplot[name path=CF-OT-MeanD-line, red, solid] coordinates {
    (0, 0.9199988842010498)
    (5, 0.8707999587059021)
    (10, 0.8245999217033386)
    (15, 0.7699998617172241)
    (20, 0.7380000352859497)
    (25, 0.6818003058433533)
    (30, 0.644599974155426)
    (35, 0.6117998957633972)
    (40, 0.5626001358032227)
    (45, 0.5194001197814941)
    (50, 0.47799986600875854)
    (55, 0.4493999481201172)
    (60, 0.4151999354362488)
    (65, 0.3793998658657074)
    (70, 0.34679996967315674)
    (75, 0.31779998540878296)
    (80, 0.2794000208377838)
    (85, 0.27000004053115845)
    (90, 0.2314000129699707)
    (95, 0.2128000408411026)
    (100, 0.18200001120567322)
    (105, 0.1550000160932541)
    (110, 0.14339999854564667)
    (115, 0.12539997696876526)
    (120, 0.103799968957901)
    (125, 0.09179998189210892)
    (130, 0.06659995764493942)
    (135, 0.052399974316358566)
    (140, 0.04479997232556343)
    (145, 0.026999983936548233)
    (150, 0.02219999022781849)
    (155, 0.015399993397295475)
    (160, 0.0073999990709125996)
    (165, 0.004200000315904617)
    (170, 0.00019999999494757503)
    (175, 0.00039999998989515007)
    (180, 0.0)
    (185, 0.0)
    (190, 0.0)
    (195, 0.0)
    (200, 0.0)
};
%\addlegendentry{CF-OT}
\addplot[name path=CF-OT-MeanD-upper, red, opacity=0.3, forget plot] coordinates {
    (0, 0.9199992418289185)
    (5, 0.8784430027008057)
    (10, 0.8333247303962708)
    (15, 0.7805104851722717)
    (20, 0.750505805015564)
    (25, 0.6963729858398438)
    (30, 0.6592840552330017)
    (35, 0.6275443434715271)
    (40, 0.5766755938529968)
    (45, 0.5345945358276367)
    (50, 0.4912131428718567)
    (55, 0.46741238236427307)
    (60, 0.4323161840438843)
    (65, 0.39626970887184143)
    (70, 0.3632212281227112)
    (75, 0.33367598056793213)
    (80, 0.29734015464782715)
    (85, 0.2850237488746643)
    (90, 0.24816164374351501)
    (95, 0.2286657989025116)
    (100, 0.19588474929332733)
    (105, 0.16820919513702393)
    (110, 0.1566641628742218)
    (115, 0.1373877078294754)
    (120, 0.11530227959156036)
    (125, 0.10249831527471542)
    (130, 0.07623106986284256)
    (135, 0.0609707348048687)
    (140, 0.05231153219938278)
    (145, 0.03380049765110016)
    (150, 0.02785399928689003)
    (155, 0.02065364643931389)
    (160, 0.01119878701865673)
    (165, 0.006880904082208872)
    (170, 0.0008549000485800207)
    (175, 0.0013214806094765663)
    (180, 0.0)
    (185, 0.0)
    (190, 0.0)
    (195, 0.0)
    (200, 0.0)
};
\addplot[name path=CF-OT-MeanD-lower, red, opacity=0.3, forget plot] coordinates {
    (0, 0.9199985265731812)
    (5, 0.8631569147109985)
    (10, 0.8158751130104065)
    (15, 0.7594892382621765)
    (20, 0.7254942655563354)
    (25, 0.6672276258468628)
    (30, 0.6299158930778503)
    (35, 0.5960554480552673)
    (40, 0.5485246777534485)
    (45, 0.5042057037353516)
    (50, 0.4647865891456604)
    (55, 0.4313875138759613)
    (60, 0.3980836868286133)
    (65, 0.36253002285957336)
    (70, 0.3303787112236023)
    (75, 0.3019239902496338)
    (80, 0.2614598870277405)
    (85, 0.2549763321876526)
    (90, 0.2146383821964264)
    (95, 0.1969342827796936)
    (100, 0.1681152731180191)
    (105, 0.14179083704948425)
    (110, 0.13013583421707153)
    (115, 0.11341223865747452)
    (120, 0.09229765832424164)
    (125, 0.08110164850950241)
    (130, 0.056968849152326584)
    (135, 0.043829213827848434)
    (140, 0.03728841245174408)
    (145, 0.020199468359351158)
    (150, 0.016545981168746948)
    (155, 0.010146339423954487)
    (160, 0.003601210657507181)
    (165, 0.0015190965496003628)
    (170, -0.00045490002958104014)
    (175, -0.0005214805714786053)
    (180, 0.0)
    (185, 0.0)
    (190, 0.0)
    (195, 0.0)
    (200, 0.0)
};
\addplot[fill opacity=0.3, red, forget plot] fill between[of=CF-OT-MeanD-upper and CF-OT-MeanD-lower];
\addplot[name path=CF_Exact-MeanD-line, black, dashed] coordinates {
    (0, 0.9199988842010498)
    (5, 0.8665997982025146)
    (10, 0.8263999223709106)
    (15, 0.7739999890327454)
    (20, 0.7395997643470764)
    (25, 0.6928001642227173)
    (30, 0.6513999104499817)
    (35, 0.6097999811172485)
    (40, 0.5778002738952637)
    (45, 0.5502001643180847)
    (50, 0.5221999883651733)
    (55, 0.48399993777275085)
    (60, 0.4627997577190399)
    (65, 0.43899983167648315)
    (70, 0.4109998643398285)
    (75, 0.39939987659454346)
    (80, 0.3723999857902527)
    (85, 0.35819992423057556)
    (90, 0.34359991550445557)
    (95, 0.32439985871315)
    (100, 0.30559998750686646)
    (105, 0.2943999171257019)
    (110, 0.283799946308136)
    (115, 0.2600000202655792)
    (120, 0.2547999620437622)
    (125, 0.25)
    (130, 0.25039997696876526)
    (135, 0.24319995939731598)
    (140, 0.23020000755786896)
    (145, 0.21480000019073486)
    (150, 0.21899999678134918)
    (155, 0.2038000226020813)
    (160, 0.20400004088878632)
    (165, 0.1972000151872635)
    (170, 0.20120005309581757)
    (175, 0.19880002737045288)
    (180, 0.18059998750686646)
    (185, 0.18500001728534698)
    (190, 0.17760004103183746)
    (195, 0.1714000254869461)
    (200, 0.16540002822875977)
};
%\addlegendentry{CF_Exact}
\addplot[name path=Optimal-MeanD-line, black, solid] coordinates {
    (0, 0.9200000000000005)
    (5, 0.82)
    (10, 0.7199999999999999)
    (15, 0.6199999999999998)
    (20, 0.5199999999999997)
    (25, 0.4199999999999997)
    (30, 0.31999999999999984)
    (35, 0.21999999999999975)
    (40, 0.11999999999999977)
    (45, 0.06)
    (50, 0.02)
    (55, 0.0)
    (60, 0.0)
    (65, 0.0)
    (70, 0.0)
    (75, 0.0)
    (80, 0.0)
    (85, 0.0)
    (90, 0.0)
    (95, 0.0)
    (100, 0.0)
    (105, 0.0)
    (110, 0.0)
    (115, 0.0)
    (120, 0.0)
    (125, 0.0)
    (130, 0.0)
    (135, 0.0)
    (140, 0.0)
    (145, 0.0)
    (150, 0.0)
    (155, 0.0)
    (160, 0.0)
    (165, 0.0)
    (170, 0.0)
    (175, 0.0)
    (180, 0.0)
    (185, 0.0)
    (190, 0.0)
    (195, 0.0)
    (200, 0.0)
};
%\addlegendentry{Optimal}
\end{axis}
\end{tikzpicture}



==> pictures/german_credit_optimality/lightgbm_KNN.tex <==

\begin{tikzpicture}
\begin{axis}[
    width=4.4cm, height=3.6cm,
    legend pos=north east,
    legend style={
        draw=none,
        % font=\scriptsize,
        legend image code/.code={
            \draw[mark repeat=2,mark phase=2]
                plot coordinates {
                    (0cm,0cm)
                    (0.4cm,0cm) % Adjust the length here
                };
        },
        inner xsep=0pt, % Adjust inner x separation
        inner ysep=0pt  % Adjust inner y separation
    },
    legend cell align={left},
    grid=major,
    title={LightGBM, $\A_{\text{CE}}=$KNN},
    title style={font=\footnotesize, yshift=-1ex}, 
    font=\footnotesize,
    % Increase margin of x and y tick labels
    xticklabel style={xshift=-0pt, yshift=-3pt},
    yticklabel style={xshift=-3pt, yshift=0pt},
]
        \addplot[name path=CF-OT-MeanD-line, red, solid] coordinates {
    (0, 0.7999999999999985)
    (5, 0.7428000000000001)
    (10, 0.689)
    (15, 0.6347999999999999)
    (20, 0.5838)
    (25, 0.5312)
    (30, 0.48180000000000023)
    (35, 0.44260000000000005)
    (40, 0.3860000000000002)
    (45, 0.3498000000000001)
    (50, 0.31680000000000014)
    (55, 0.26799999999999996)
    (60, 0.23919999999999994)
    (65, 0.19679999999999997)
    (70, 0.17059999999999992)
    (75, 0.14079999999999995)
    (80, 0.11259999999999992)
    (85, 0.09839999999999995)
    (90, 0.07259999999999997)
    (95, 0.06519999999999995)
    (100, 0.04899999999999999)
    (105, 0.03620000000000003)
    (110, 0.02740000000000002)
    (115, 0.021000000000000015)
    (120, 0.016400000000000012)
    (125, 0.015000000000000012)
    (130, 0.012400000000000007)
    (135, 0.01320000000000001)
    (140, 0.010400000000000006)
    (145, 0.009400000000000006)
    (150, 0.006800000000000004)
    (155, 0.004600000000000002)
    (160, 0.0030000000000000005)
    (165, 0.0020000000000000005)
    (170, 0.0001999999999999999)
    (175, 0.0)
    (180, 0.0)
    (185, 0.0)
    (190, 0.0)
    (195, 0.0)
    (200, 0.0)
};
%\addlegendentry{CF-OT}
\addplot[name path=CF-OT-MeanD-upper, red, opacity=0.3, forget plot] coordinates {
    (0, 0.799999999999999)
    (5, 0.7497669778218107)
    (10, 0.7004902568026132)
    (15, 0.6467066906408792)
    (20, 0.5976596041048653)
    (25, 0.5454487758686001)
    (30, 0.4972948444372832)
    (35, 0.4595262372098586)
    (40, 0.40099483036116135)
    (45, 0.36781340807530893)
    (50, 0.3355724363391011)
    (55, 0.28412254148699884)
    (60, 0.2567609930961093)
    (65, 0.21159764765716493)
    (70, 0.18438940781572571)
    (75, 0.15620581744541973)
    (80, 0.12704010397761725)
    (85, 0.11219647491812305)
    (90, 0.0854190258757988)
    (95, 0.07688634053660935)
    (100, 0.061809559600157986)
    (105, 0.04501570386206345)
    (110, 0.034589460480759344)
    (115, 0.02720071911555428)
    (120, 0.021777941106259913)
    (125, 0.01930354092695772)
    (130, 0.016324991803099726)
    (135, 0.016831451112929937)
    (140, 0.013688366146036666)
    (145, 0.012814402587335015)
    (150, 0.00991795113265106)
    (155, 0.00736991956930161)
    (160, 0.005350244095833453)
    (165, 0.003974600000000002)
    (170, 0.0008549007311035754)
    (175, 0.0)
    (180, 0.0)
    (185, 0.0)
    (190, 0.0)
    (195, 0.0)
    (200, 0.0)
};
\addplot[name path=CF-OT-MeanD-lower, red, opacity=0.3, forget plot] coordinates {
    (0, 0.7999999999999979)
    (5, 0.7358330221781896)
    (10, 0.6775097431973867)
    (15, 0.6228933093591207)
    (20, 0.5699403958951347)
    (25, 0.5169512241313999)
    (30, 0.46630515556271723)
    (35, 0.4256737627901415)
    (40, 0.371005169638839)
    (45, 0.3317865919246913)
    (50, 0.29802756366089916)
    (55, 0.2518774585130011)
    (60, 0.2216390069038906)
    (65, 0.18200235234283502)
    (70, 0.15681059218427412)
    (75, 0.12539418255458018)
    (80, 0.09815989602238258)
    (85, 0.08460352508187684)
    (90, 0.05978097412420114)
    (95, 0.05351365946339055)
    (100, 0.03619044039984199)
    (105, 0.027384296137936606)
    (110, 0.020210539519240702)
    (115, 0.01479928088444575)
    (120, 0.01102205889374011)
    (125, 0.010696459073042305)
    (130, 0.008475008196900287)
    (135, 0.009568548887070085)
    (140, 0.007111633853963348)
    (145, 0.005985597412664996)
    (150, 0.003682048867348948)
    (155, 0.0018300804306983936)
    (160, 0.0006497559041665486)
    (165, 2.5399999999998774e-05)
    (170, -0.00045490073110357563)
    (175, 0.0)
    (180, 0.0)
    (185, 0.0)
    (190, 0.0)
    (195, 0.0)
    (200, 0.0)
};
\addplot[fill opacity=0.3, red, forget plot] fill between[of=CF-OT-MeanD-upper and CF-OT-MeanD-lower];
\addplot[name path=CF_Exact-MeanD-line, black, dashed] coordinates {
    (0, 0.7999999999999985)
    (5, 0.7580000000000002)
    (10, 0.7143999999999997)
    (15, 0.6781999999999998)
    (20, 0.6365999999999998)
    (25, 0.5925999999999996)
    (30, 0.5704)
    (35, 0.5332)
    (40, 0.5027999999999999)
    (45, 0.4680000000000002)
    (50, 0.44100000000000017)
    (55, 0.41020000000000023)
    (60, 0.3972000000000001)
    (65, 0.35320000000000024)
    (70, 0.32719999999999994)
    (75, 0.31320000000000003)
    (80, 0.2922000000000002)
    (85, 0.25680000000000003)
    (90, 0.23919999999999983)
    (95, 0.2201999999999999)
    (100, 0.21379999999999985)
    (105, 0.19579999999999995)
    (110, 0.1764)
    (115, 0.17059999999999995)
    (120, 0.15959999999999994)
    (125, 0.11999999999999991)
    (130, 0.1221999999999999)
    (135, 0.11219999999999991)
    (140, 0.09739999999999999)
    (145, 0.08539999999999996)
    (150, 0.07699999999999994)
    (155, 0.06879999999999993)
    (160, 0.06139999999999996)
    (165, 0.05359999999999996)
    (170, 0.04280000000000002)
    (175, 0.040400000000000026)
    (180, 0.03400000000000002)
    (185, 0.031000000000000017)
    (190, 0.026800000000000015)
    (195, 0.02620000000000002)
    (200, 0.022000000000000016)
};
%\addlegendentry{CF_Exact}
\addplot[name path=Optimal-MeanD-line, black, solid] coordinates {
    (0, 0.7999999523162842)
    (5, 0.7)
    (10, 0.6)
    (15, 0.5)
    (20, 0.4)
    (25, 0.3)
    (30, 0.19999999999999998)
    (35, 0.1)
    (40, 0.04)
    (45, 0.0)
    (50, 0.0)
    (55, 0.0)
    (60, 0.0)
    (65, 0.0)
    (70, 0.0)
    (75, 0.0)
    (80, 0.0)
    (85, 0.0)
    (90, 0.0)
    (95, 0.0)
    (100, 0.0)
    (105, 0.0)
    (110, 0.0)
    (115, 0.0)
    (120, 0.0)
    (125, 0.0)
    (130, 0.0)
    (135, 0.0)
    (140, 0.0)
    (145, 0.0)
    (150, 0.0)
    (155, 0.0)
    (160, 0.0)
    (165, 0.0)
    (170, 0.0)
    (175, 0.0)
    (180, 0.0)
    (185, 0.0)
    (190, 0.0)
    (195, 0.0)
    (200, 0.0)
};
%\addlegendentry{Optimal}
\end{axis}
\end{tikzpicture}



==> pictures/german_credit_optimality/xgboost_DiCE.tex <==

\begin{tikzpicture}
\begin{axis}[
    width=4.4cm, height=3.6cm,
    legend pos=north east,
    legend style={
        draw=none,
        % font=\scriptsize,
        legend image code/.code={
            \draw[mark repeat=2,mark phase=2]
                plot coordinates {
                    (0cm,0cm)
                    (0.4cm,0cm) % Adjust the length here
                };
        },
        inner xsep=0pt, % Adjust inner x separation
        inner ysep=0pt  % Adjust inner y separation
    },
    legend cell align={left},
    grid=major,
    title={XGBoost, $\A_{\text{CE}}$=DiCE},
    title style={font=\footnotesize, yshift=-1ex}, 
    font=\footnotesize,
    % Increase margin of x and y tick labels
    xticklabel style={xshift=-0pt, yshift=-3pt},
    yticklabel style={xshift=-3pt, yshift=0pt},
]
        \addplot[name path=CF-OT-MeanD-line, red, solid] coordinates {
    (0, 0.8799999999999996)
    (5, 0.8053999999999992)
    (10, 0.7374)
    (15, 0.6743999999999994)
    (20, 0.6005999999999997)
    (25, 0.5380000000000001)
    (30, 0.49219999999999986)
    (35, 0.4288)
    (40, 0.3784)
    (45, 0.3262000000000001)
    (50, 0.2820000000000001)
    (55, 0.2403999999999998)
    (60, 0.206)
    (65, 0.16259999999999997)
    (70, 0.14319999999999997)
    (75, 0.11739999999999995)
    (80, 0.09499999999999996)
    (85, 0.07079999999999995)
    (90, 0.05639999999999998)
    (95, 0.039600000000000024)
    (100, 0.030000000000000023)
    (105, 0.021600000000000015)
    (110, 0.01760000000000001)
    (115, 0.011400000000000006)
    (120, 0.004800000000000001)
    (125, 0.0002)
    (130, 0.0)
    (135, 0.0)
    (140, 0.0)
    (145, 0.0)
    (150, 0.0)
    (155, 0.0)
    (160, 0.0)
    (165, 0.0)
    (170, 0.0)
    (175, 0.0)
    (180, 0.0)
    (185, 0.0)
    (190, 0.0)
    (195, 0.0)
    (200, 0.0)
};
\addlegendentry{CF-$p_{\text{OT}}$}
\addplot[name path=CF-OT-MeanD-upper, red, opacity=0.3, forget plot] coordinates {
    (0, 0.8799999999999997)
    (5, 0.8119061996296141)
    (10, 0.7459644441736987)
    (15, 0.6855731267547803)
    (20, 0.6125370336142776)
    (25, 0.5499386666742984)
    (30, 0.5076332110812881)
    (35, 0.4422993594749381)
    (40, 0.39440603825580833)
    (45, 0.34067127207758885)
    (50, 0.29540855341190847)
    (55, 0.2556946193319871)
    (60, 0.22052520794618788)
    (65, 0.17715961609399092)
    (70, 0.15388313549973037)
    (75, 0.1285953996268288)
    (80, 0.10538100553655566)
    (85, 0.07960217925298042)
    (90, 0.0645881773101466)
    (95, 0.04618068346833369)
    (100, 0.03488134184420639)
    (105, 0.02603296600555431)
    (110, 0.022186667066007748)
    (115, 0.015484553955133906)
    (120, 0.007611061162194808)
    (125, 0.0008549007311035771)
    (130, 0.0)
    (135, 0.0)
    (140, 0.0)
    (145, 0.0)
    (150, 0.0)
    (155, 0.0)
    (160, 0.0)
    (165, 0.0)
    (170, 0.0)
    (175, 0.0)
    (180, 0.0)
    (185, 0.0)
    (190, 0.0)
    (195, 0.0)
    (200, 0.0)
};
\addplot[name path=CF-OT-MeanD-lower, red, opacity=0.3, forget plot] coordinates {
    (0, 0.8799999999999994)
    (5, 0.7988938003703844)
    (10, 0.7288355558263014)
    (15, 0.6632268732452186)
    (20, 0.5886629663857218)
    (25, 0.5260613333257019)
    (30, 0.47676678891871155)
    (35, 0.41530064052506194)
    (40, 0.3623939617441917)
    (45, 0.31172872792241135)
    (50, 0.2685914465880917)
    (55, 0.2251053806680125)
    (60, 0.1914747920538121)
    (65, 0.14804038390600902)
    (70, 0.13251686450026956)
    (75, 0.10620460037317109)
    (80, 0.08461899446344426)
    (85, 0.06199782074701947)
    (90, 0.048211822689853356)
    (95, 0.03301931653166636)
    (100, 0.025118658155793658)
    (105, 0.01716703399444572)
    (110, 0.013013332933992275)
    (115, 0.007315446044866105)
    (120, 0.001988938837805195)
    (125, -0.00045490073110357715)
    (130, 0.0)
    (135, 0.0)
    (140, 0.0)
    (145, 0.0)
    (150, 0.0)
    (155, 0.0)
    (160, 0.0)
    (165, 0.0)
    (170, 0.0)
    (175, 0.0)
    (180, 0.0)
    (185, 0.0)
    (190, 0.0)
    (195, 0.0)
    (200, 0.0)
};
\addplot[fill opacity=0.3, red, forget plot] fill between[of=CF-OT-MeanD-upper and CF-OT-MeanD-lower];
\addplot[name path=CF_Exact-MeanD-line, black, dashed] coordinates {
    (0, 0.8799999999999996)
    (5, 0.7927999999999998)
    (10, 0.7070000000000004)
    (15, 0.6183999999999998)
    (20, 0.5324000000000002)
    (25, 0.4484000000000003)
    (30, 0.36939999999999984)
    (35, 0.28580000000000044)
    (40, 0.2041999999999998)
    (45, 0.12799999999999992)
    (50, 0.06459999999999995)
    (55, 0.01800000000000001)
    (60, 0.0014000000000000002)
    (65, 0.0)
    (70, 0.0)
    (75, 0.0)
    (80, 0.0)
    (85, 0.0)
    (90, 0.0)
    (95, 0.0)
    (100, 0.0)
    (105, 0.0)
    (110, 0.0)
    (115, 0.0)
    (120, 0.0)
    (125, 0.0)
    (130, 0.0)
    (135, 0.0)
    (140, 0.0)
    (145, 0.0)
    (150, 0.0)
    (155, 0.0)
    (160, 0.0)
    (165, 0.0)
    (170, 0.0)
    (175, 0.0)
    (180, 0.0)
    (185, 0.0)
    (190, 0.0)
    (195, 0.0)
    (200, 0.0)
};
\addlegendentry{CF-$p_{\text{Ect}}$}
\addplot[name path=Optimal-MeanD-line, black, solid] coordinates {
    (0, 0.88)
    (5, 0.7799999999999999)
    (10, 0.6800000000000003)
    (15, 0.5800000000000002)
    (20, 0.48000000000000015)
    (25, 0.38000000000000006)
    (30, 0.27999999999999997)
    (35, 0.18)
    (40, 0.08)
    (45, 0.04)
    (50, 0.0)
    (55, 0.0)
    (60, 0.0)
    (65, 0.0)
    (70, 0.0)
    (75, 0.0)
    (80, 0.0)
    (85, 0.0)
    (90, 0.0)
    (95, 0.0)
    (100, 0.0)
    (105, 0.0)
    (110, 0.0)
    (115, 0.0)
    (120, 0.0)
    (125, 0.0)
    (130, 0.0)
    (135, 0.0)
    (140, 0.0)
    (145, 0.0)
    (150, 0.0)
    (155, 0.0)
    (160, 0.0)
    (165, 0.0)
    (170, 0.0)
    (175, 0.0)
    (180, 0.0)
    (185, 0.0)
    (190, 0.0)
    (195, 0.0)
    (200, 0.0)
};
\addlegendentry{Optimal}
\end{axis}
\end{tikzpicture}



==> pictures/problem_illustration.tex <==
\begin{minipage}{0.22\textwidth}
\centering
$\vec{x}$ \\
\begin{tabular}{|c|c|c|}
\hline
\faMoney & \faMousePointer & \faRegistered \\
\hline
200 & 5 & No \\
150 & 3 & No \\
100 & 2 & No \\
150 & 6 & No \\
\hline
\end{tabular}
\end{minipage}
\quad % spacing between tables
\begin{minipage}{0.22\textwidth}
\centering
$\vec{z}'$ \\
\begin{tabular}{|c|c|c|}
\hline
\faMoney & \faMousePointer & \faRegistered \\
\hline
\bwcell{250} & \bwcell{8} & \textbf{Yes} \\
150 & 3 & No \\
\bwcell{350} & \bwcell{9} & \textbf{Yes} \\
150 & 6 & No \\
\hline
\end{tabular}
\end{minipage}
\quad % spacing between tables
\begin{minipage}{0.22\textwidth}
\centering
$\vec{z}''$ \\
\begin{tabular}{|c|c|c|}
\hline
\faMoney & \faMousePointer & \faRegistered \\
\hline
200 & 5 & No \\
150 & \bwcell{7} & \textbf{Yes} \\
100 & 2 & No \\
\bwcell{350} & 6 & \textbf{Yes} \\
\hline
\end{tabular}
\end{minipage}
\quad % spacing between tables
\begin{minipage}{0.12\textwidth}
\centering
$\vec{y}^*$ \\
\begin{tabular}{|c|}
\hline
\faRegistered \\
\hline
Yes \\
Yes\\
Yes \\
Yes \\
\hline
\end{tabular}
\end{minipage}
